Faster Lattice Basis Computation via a Natural Generalization of the Euclidean Algorithm

The Euclidean algorithm is the oldest algorithms known to mankind. Given two integral numbers $a_1$ and $a_2$, it computes the greatest common divisor (gcd) of $a_1$ and $a_2$ in a very elegant way. From a lattice perspective, it computes a basis of the sum of two one-dimensional lattices $a_1 \mathbb{Z}$ and $a_2 \mathbb{Z}$ as $\gcd(a_1,a_2) \mathbb{Z} = a_1 \mathbb{Z} + a_2 \mathbb{Z}$. In this paper, we show that the classical Euclidean algorithm can be adapted in a very natural way to compute a basis of a general lattice $L(A_1, \ldots , A_n)$ given vectors $A_1, \ldots , A_n \in \mathbb{Z}^d$ with $n> \mathrm{rank}(a_1, \ldots ,a_d)$. Similar to the Euclidean algorithm, our algorithm is very easy to describe and implement and can be written within 12 lines of pseudocode. As our main result, we obtain an algorithm to compute a lattice basis for given vectors $A_1, \ldots , A_n \in \mathbb{Z}^d$ in time (counting bit operations) $LS + \tilde{O}((n-d)d^2 \cdot \log(||A||)$, where $LS$ is the time required to obtain the exact fractional solution of a certain system of linear equalities. The analysis of the running time of our algorithms relies on fundamental statements on the fractionality of solutions of linear systems of equations. So far, the fastest algorithm for lattice basis computation was due to Storjohann and Labhan [SL96] having a running time of $\tilde{O}(nd^\omega\log ||A||)$. For current upper bounds of $LS$, our algorithm has a running time improvement of a factor of at least $d^{0.12}$ over [SL96]. Our algorithm is therefore the first general algorithmic improvement to this classical problem in nearly 30 years. At last, we present a postprocessing procedure which yields an improved size bound of $\sqrt{d} ||A||$ for vectors of the resulting basis matrix.

==> abstract <==
The Euclidean algorithm is one of the oldest algorithms known to mankind. Given two integral numbers a and b , it computes the greatest common divisor (gcd) of a and b in a very elegant way. From a lattice perspective, it computes a basis of the sum of two one-dimensional lattices a Z and b Z as gcd(a , b)Z = a Z + b Z. In this paper, we show that the classical Euclidean algorithm can be adapted in a very natural way to compute a basis of a general lattice L(a_1 ,. .. , a_m) given vectors a_1 , ... , a_m ∈ Z n with m > rank(a_1 ,. .. , a_m). Similar to the Euclidean algorithm, our algorithm is very easy to describe and implement and can be written within 12 lines of pseudocode. While the Euclidean algorithm halves the largest number in every iteration, our generalized algorithm halves the determinant of a full rank subsystem leading to at most log(det B) many iterations, for some initial subsystem B. Therefore, we can compute a basis of the lattice using at most Õ((m−n)n log(det B)+mn ^(ω−1) log(||A||_∞)) arithmetic operations, where ω is the matrix multiplication exponent and A = (a_1 ,. .. , a_m). Even using the worst case Hadamard bound for the determinant, our algorithm improves upon existing algorithm. Another major advantage of our algorithm is that we can bound the entries of the resulting lattice basis by O(n^2 · ||A||_∞) using a simple pivoting rule. This is in contrast to the typical approach for computing lattice basis, where the Hermite normal form (HNF) is used. In the HNF, entries can be as large as the determinant and hence can only be bounded by an exponential term.







The Euclidean algorithm the oldest algorithms known to mankind. Given two integral numbers $a_1$ and $a_2$, it computes the greatest common divisor (gcd) of $a_1$ and $a_2$ in a very elegant way. From a lattice perspective, it computes a basis of the sum of two one-dimensional lattices $a_1 \mathbb{Z}$ and $a_2 \mathbb{Z}$ as $\gcd(a_1,a_2) \mathbb{Z} = a_1 \mathbb{Z} + a_2 \mathbb{Z}$. In this paper, we show that the classical Euclidean algorithm can be adapted in a very natural way to compute a basis of a general lattice $L (A_1, \ldots , A_n)$ given vectors $A_1, \ldots , A_n \in \mathbb{Z}^d$ with $n> \mathrm{rank}(a_1, \ldots ,a_d)$. Similar to the Euclidean algorithm, our algorithm is very easy to describe and implement and can be written within 12 lines of pseudocode.
  Our generalized version of the Euclidean algorithm allows for several degrees of freedom in the pivoting process. Hence, in a second step, we show that this freedom can be exploited to make the algorithm perform more efficiently. As our main result, we obtain an algorithm to compute a lattice basis for given vectors $A_1, \ldots , A_n \in \mathbb{Z}^d$ in time (counting bit operations) $LS + \tilde O ((n-d)d^2 \cdot \log(||A||)$, where $LS$ is the time required to obtain the exact fractional solution of a certain system of linear equalities. The analysis of the running time of our algorithms relies on fundamental statements on the fractionality of solutions of linear systems of equations.
  So far, the fastest algorithm for lattice basis computation was due to Storjohann and Labhan [SL96] having a running time of $\tilde O (nd^\omega\log ||A||)$. For current upper bounds of $LS$, our algorithm has a running time improvement of a factor of at least $d^{0.12}$ over [SL96]. Our algorithm is therefore the first general algorithmic improvement to this classical problem in nearly 30 years.

==> old_specialcase.tex <==
\subsection{Case $m=n+1$}

\begin{comment}
Find a maximal linearly independent set of vectors:
\begin{itemize}
    \item Randomized algorithm in $\OTilde(nnz(A) + r^\omega)$ field operations~\cite{DBLP:journals/jacm/CheungKL13}. More expensive in bit operations? BUT maybe we can use randomization in the p-adic style to remain this running time? Field operations in running time $\OTilde(\log n +\log |F|)$.
    \item \cite{DBLP:journals/jal/IbarraMH82} find maximal subset of linearly independent vectors modulo a given prime $p$ in time $O(mn^{\omega-1})$. Can we guess suitable prime in same way as the Las Vegas algorithms? Actually we should be able to use the same prime for both occasions.
\end{itemize}
\end{comment}

Denote with $B(t)$ the time required to perform multiplication and gcd-like operations on $t$ bit integers and $MM(n)$ the time required to do matrix multiplication of dimension $n$ over a ring.
\begin{theorem}[\cite{DBLP:journals/jc/Storjohann05}]
Let a full column rank $B\in\zz^{n\times m}$ be given. A prime $p$ with $\log p = O(\log m + \log \log \norm{B})$ together with a permutation matrix $P$ such that the principal $m\times m$ submatrix of $PB \mod p$ is nonsingular over $\zz / p$ can be found with an expected number of \[O(n\log n MM(m)/m \cdot B(\log\norm{B}+\log m))\] bit operations.  
\end{theorem}
Transpose the matrix, then this is also possible for full row rank. If row rank is not full, should also be possible because they derive the below statement (so they should be able to do so). Running time in our case is $\OTilde(n(n+1)^{\omega -1}\log\norm{A})$. 
\begin{theorem}[\cite{DBLP:journals/jc/Storjohann05}]
Let $A\in\zz^{n\times m}$ and $b\in\zz^n$ be given. There exists a Las Vegas algorithm that either proves that $Ax=b$ has no rational solution vector or computes a solution with minimum denominator  with an expected number of 
\[nm\log r (MM(r)/r^2)B(\max\{\log\norm{A}, \log\norm{b}/r\}+\log m)\]
bit operations, where $r$ is the rank of $A$.
\end{theorem}
This is in our case in $\OTilde((n+1)n^{\omega-1}\log^2 \norm A)$.

Given the initial solution $x$ for $Ax=b$ we proceed similar to lines $8-10$ in Algorithm~\ref{alg:easyversion}. %The updated solution can be calculated by 
%\[x_j' := x_j / x_i \text{ if $i\neq j$ and } x_i' := 1/x_i.\]
The update step requires at most $n$ arithmetic operations. \todo{Numbers bounded by... so this is at most ... bit operations. Matrix infinity norm can grow up to $n\norm{A}_\infty$, eventually we need an additional operation modulo the initial base in every iteration. }

In this case we have an expected running time of roughly 
\[\OTilde(n^\omega \log^2\norm{A}_\infty + n\cdot \log^2(\text{det}_{\max})\log\norm{A}_\infty) \leq \OTilde(n^3\log^2\norm{A}_\infty).\]


\section{Refinements -- Otherwise Known as \emph{The Lazy Version}}
\todo{SOLUTION UPDATES TOO SLOW.}


\subsection{Algorithm}

Since almost every nice-to-have operation is too expensive to compute, in Algorithm~\autoref{alg:refinedversion} we will be very very very lazy. Computing the current basis is too expensive? Then we do not keep track of the current basis $A^{(i)}$. Choosing the best update step (closest value to an integer) does not give us the desired complexity? Then we take any value that does. 

The golden rule: \emph{Never} compute a matrix-vector product if not absolutely necessary. Instead we keep track of the vectors and update them. Also we can not simply keep track of the vectors for all columns $m$ as every row undergoes essentially the same multiplications until it is chosen for an update step. So we keep track of updates per row and (for those columns that participated in an update) the multiplier up to that update, so that (full multiplier / update multiplier) leads to the correct multiplier for that row and column, see also comment $(*^2)$.

The reconstruction can only be done in desired time, if we avoid the "combination of combination"-problem. Therefore we ensure integral numbers row by row.

\todo{$s$ and $t$ need rework. However, this could simplify bit length analysis.}

\begin{algorithm}
  \caption{Generalized Euclidean Algorithm
    \label{alg:refinedversion}}
  \begin{algorithmic}[1]
    \Statex{\textsc{Input: } $a_1,\ldots, a_m \in \zz^n$ }
    \Let{$s$}{$\mathds{1}\in \qq^{n\times (m-n)}$} \Comment{Multiplication corrector for each row and column}
    \Let{$t$}{$\mathds{1}\in \qq^{n}$} \Comment{Solution update multipliers for each row} %\Comment{Which $\bar{a}_k$ or updated basis vector is the currently in this column.}
    \Let{$Y$}{$I_n$}
    \Let{$j$}{$1$}
    \State{\textbf{find} lin. ind. vectors $\bar{a}_1, \ldots, \bar{a}_n \in \{a_1,\ldots, a_m\}$ using \autoref{lem:maximal_subsystem}}
    \Let{$A^{(1)}$}{$(\bar{a}_1, \ldots, \bar{a}_n)$}
    \Let{$B$}{$\{a_1,\ldots, a_m\}\setminus \{\bar{a}_1, \ldots, \bar{a}_n\}$}
    \State{\textbf{solve} $A^{(1)}X=B$ using \autoref{theorem:system_solving_for_right-hand_side_matrix} and \autoref{lem:rational_reconstruction}}
    \While{$j\leq n$}\Comment{Goal: Integral values for all $X_{j*}$}
    \State{Choose any $1\leq \ell\leq m$ such that $(t_k-s_{k\ell}) + X_{j\ell}$ is not integral yet. }
    \State{If none exists set $j \leftarrow j+1$ and repeat line 11.}
    \State{Compute updated solution $x_k = (t_k-s_{k\ell}) +X_{k\ell}$ }
    \State{$v_k := \{x_k\}$ if $k\neq j$ and $v_j := -(x_j - \nint{x_j})$.}\Comment{Comment $(*^1)$}
    \State{%For all $1\leq k\leq n$ set
    $Y_{kj} := \{v_k \cdot Y_{kj}\}$ if $k<j$ and $Y_{kj} := \{\{x_k\} + v_k \cdot Y_{kj}\}$ otherwise}\Comment{$A^{(i)} = A^{(1)}Y$, see $(*^2)$}
    %\Comment{Representation of the update}
    \Let{$X_{*j}$}{$e_j$} %\Comment{Save solution of $j$th basis vector.}
    \Let{$s_{*\ell}$}{$t$} \Comment{Update multiplication corrector}
    \State{$t_j\leftarrow - \frac{t_j}{x_j - \nint{x_j}} $ and $t_k \leftarrow t_k\cdot (1+\frac{\{x_k\}}{x_j - \nint{x_j}})$ for all $j<k\leq n$} \Comment{Update solutions}
    \EndWhile
    \Let{$B$}{$A^{(1)}Y$} %\Comment{Compute basis by matrix-matrix-multiplication because that is faster. }
    \State \Return{$(B,Y)$} 
  \end{algorithmic}
\end{algorithm}
Comment $(*^1)$: Imitate update step $r^{(i)} := \sum_{k\neq j}A^{(i)}_k\{x_k\} - A^{(i)}_j(x_j-\nint{x_j})$, but we do not compute the updated basis vector $r^{(i)}$. Instead we only compute the representations and store the representation of the $j^{th}$ basis vector as $Y_{*j}$. 

Comment $(*^2)$: We compute $y$ such that the new basis vector $A^{(i+1)}_j=A^{(1)}y$ as follows
\begin{align*}
    A^{(i+1)}_j = &\sum_{k\neq j}A^{(i)}_k\{x^{(i)}_k\} - A^{(i)}_j(x^{(i)}_j -\nint{x^{(i)}_j})\\
    \stackrel{\{x^{(i)}_k\}=0 \text{ f.a. } k<j}{=} & \sum_{k> j}A^{(i)}_k\{x^{(i)}_k\} - A^{(i)}_j(x^{(i)}_j -\nint{x^{(i)}_j})\\
    \stackrel{A^{(i)}_k = A^{(1)}_k \text{ f.a. } k>j}{=} & \sum_{k> j}A^{(1)}_k\{x^{(i)}_k\} - A^{(i)}_j(x^{(i)}_j -\nint{x^{(i)}_j}) \\
    \stackrel{A^{(i)}_j = A^{(1)}u^{(i-1)}}{=} & \sum_{k> j}A^{(1)}_k\{x^{(i)}_k\} - (x^{(i)}_j -\nint{x^{(i)}_j}) \cdot A^{(1)}y_{\mathrm{prev}} \\
    \stackrel{y \text{ def. appr.}}{=}& A^{(1)}y
\end{align*}
Since $\{x_k\}=0$ for all $k<j$ we do not need to consider representations of $A^{(i)}_k$ in terms of $A^{(1)}$. Moreover, we alter the columns of the basis one by one. This implies the $A^{(i)}_k = A^{(1)}_k$ for all $k>j$. Hence only the representation of $A^{(i)}_j$ needs to be tracked, and is stored in the previous $u$. It is, however, very necessary for our running time that we do not perform the matrix-vector multiplication to compute the basis vector directly. Instead, we will do this for all basis vectors at once using matrix-matrix multiplication in the last rows. Moreover, we only ever store the fractional part. Hence every new basis vector is in the fundamental parallelopiped of $A^{(1)}$ and is therefore bounded by $n\norm{A}_\infty$ in $\ell_\infty$-norm.


\subsection{Running Time}
\begin{itemize}
    \item Lines $1-8$ can be computed in time $\OTilde(mn^{\omega-1}\log\norm{A}_\infty + n^{\omega}\log\norm{A}_\infty + (m-n) n^{2.251640}\log\norm{A}_\infty)$.
    \item  (The while loop has at most $\log\det(A^{(1)}) \in O(n\log(n\norm{A}_\infty))$ iterations.)
    \item In lines $10-11$ searches each row $X_{j*}$ without finding a non-integral value at most once.  Hence it requires $\OTilde(mn \cdot M(\text{bitlength bound}) + n\log(n\norm{A}_\infty)\cdot m \cdot M(\text{bitlength bound}))$.
    \item Lines $12-17$ each involve at most $O(n)$ arithmetic operations. Hence, the running time is $\OTilde(n \cdot n\log(n\norm{A}_\infty) \cdot M(\text{bitlength bound})) = \OTilde(n^2\log\norm{A}_\infty \cdot M(\text{bitlength bound}))$ bit operations.
    \item Line $18$  is a matrix multiplication and can be computed in $\OTilde(n^{\omega}\cdot  M(\text{bitlength bound}))$.
\end{itemize}

If we can bound the bitlengths involved by some function in $O((n\log\norm{A}_\infty)^{1+\epsilon})$, then our overall complexity is 
\[\OTilde((m-n) n^{2.251640}\log\norm{A}_\infty +  n^{\omega+1}\log\norm{A}_\infty + n^3\log^2\norm{A}_\infty).\]
\todo{We have to check the involved bit-length. All the bookkeeping and multiplications might do unexpected things.\\
However, i think the denominators should always be $\leq \det(A^{(1)})$ and nominators only large if we are also doing a good improvement. Maybe we will need to analyse bitlength and number of iterations together.}

\subsubsection{Bitlength Bound}
\begin{itemize}
    \item Bound for $v$ is less or equal to bounds for $t$
    \item Matrix $X$ is solution matrix and changes only to
\end{itemize}



==> short_abstract.tex <==
The Euclidean algorithm is the oldest algorithms known to mankind. Given two integral numbers $a_1$ and $a_2$, it computes the greatest common divisor (gcd) of $a_1$ and $a_2$ in a very elegant way. From a lattice perspective, it computes a basis of the sum of two one-dimensional lattices $a_1 \mathbb{Z}$ and $a_2 \mathbb{Z}$ as $\gcd(a_1,a_2) \mathbb{Z} = a_1 \mathbb{Z} + a_2 \mathbb{Z}$. In this paper, we show that the classical Euclidean algorithm can be adapted in a very natural way to compute a basis of a general lattice $\mathcal{L}(A_1, \ldots , A_n)$ given vectors $A_1, \ldots , A_n \in \mathbb{Z}^d$ with $n> \mathrm{rank}(a_1, \ldots ,a_d)$. Similar to the Euclidean algorithm, our algorithm is very easy to describe and implement and can be written within 12 lines of pseudocode.

Our generalized version of the Euclidean algorithm allows for several degrees of freedom in the pivoting process. Hence, in a second step, we show that this freedom can be exploited to make the algorithm perform more efficiently. As our main result, we obtain an algorithm to compute a lattice basis for given vectors $A_1, \ldots , A_n \in \mathbb{Z}^d$ in time (counting bit operations) $LS + \Tilde{O}((n-d)d^2 \cdot \log(||A||)$, where $LS$ is the time required to obtain the exact fractional solution of a certain system of linear equalities.
The analysis of the running time of our algorithms relies on fundamental statements on the fractionality of solutions of linear systems of equations. 

So far, the fastest algorithm for lattice basis computation was due to Storjohann and Labhan [SL96] having a running time of $\tilde{O}(nd^\omega\log ||A||)$. For current upper bounds of $LS$, our algorithm has a running time improvement of a factor of at least $d^{0.12}$ over [SL96]. Our algorithm is therefore the first general algorithmic improvement to this classical problem in nearly 30 years.
